SemRob: Towards Semantic Stream Reasoning for Robotic Operating Systems

Stream processing and reasoning is getting considerable attention in various application domains such as IoT, Industry IoT and Smart Cities. In parallel, reasoning and knowledge-based features have attracted research into many areas of robotics, such as robotic mapping, perception and interaction. To this end, the Semantic Stream Reasoning (SSR) framework can unify the representations of symbolic/semantic streams with deep neural networks, to integrate high-dimensional data streams, such as video streams and LiDAR point clouds, with traditional graph or relational stream data. As such, this positioning and system paper will outline our approach to build a platform to facilitate semantic stream reasoning capabilities on a robotic operating system called SemRob.

==> ref-full.tex <==
@inproceedings{Suchan:2019,
  title     = {Out of Sight But Not Out of Mind: An Answer Set Programming Based Online Abduction Framework for Visual Sensemaking in Autonomous Driving},
  author    = {Suchan, Jakob and Bhatt, Mehul and Varadarajan, Srikrishna},
  booktitle = {{IJCAI-19}},          
  pages     = {1879--1885},
  year      = {2019},
}

@article{Le-Phuoc:2021,
author  = {Le-Phuoc, Danh and Eiter, Thomas and Le-Tuan, Anh},
title   = {{A Scalable Reasoning and Learning Approach for Neural-Symbolic Stream Fusion}},
journal = {AAAI'21},
year    = {2021}
}

@inproceedings{Michael:2018,
  author    = {Michael Beetz and
               Daniel Be{\ss}ler and
               Andrei Haidu and
               Mihai Pomarlan and
               Asil Kaan Bozcuoglu and
               Georg Bartels},
  title     = {Know Rob 2.0 - {A} 2nd Generation Knowledge Processing Framework for
               Cognition-Enabled Robotic Agents},
  booktitle = {2018 {IEEE}, {ICRA}
               2018},
  pages     = {512--519},
  year      = {2018},
}



@article{Sourav:2020,
  author    = {Sourav Garg and
               Niko S{\"{u}}nderhauf and
               Feras Dayoub and
               Douglas Morrison and
               Akansel Cosgun and
               Gustavo Carneiro and
               Qi Wu and
               Tat{-}Jun Chin and
               Ian D. Reid and
               Stephen Gould and
               Peter Corke and
               Michael Milford},
  title     = {Semantics for Robotic Mapping, Perception and Interaction: {A} Survey},
  journal   = {Found. Trends Robotics},
  volume    = {8},
  number    = {1-2},
  pages     = {1--224},
  year      = {2020},
}

@inproceedings{Lyu:2019,
  title={SDRL: interpretable and data-efficient deep reinforcement learning leveraging symbolic planning},
  author={Lyu, Daoming and Yang, Fangkai and Liu, Bo and Gustafson, Steven},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  pages={2970--2977},
  year={2019}
}

@ARTICLE{Illanes:2020,
  title    = "Symbolic plans as high-level instructions for reinforcement
              learning",
  author   = "Illanes, Le{\'o}n and Yan, Xi and Icarte, Rodrigo Toro and
              McIlraith, Sheila A",
  journal  = "Proceedings International Conference on Automated Planning and
              Scheduling, ICAPS 2019",
  volume   =  30,
  number   = "Icaps",
  pages    = "540--550",
  year     =  2020
}

@inproceedings{Le-Phuoc2018-b,
author="Le-Phuoc, Danh
and Xavier Parreira, Josiane 
and Hauswirth, Manfred",
editor="Liu, Ling and Azsu, M. Tamer",
title={Semantic Streams},
booktitle={Encyclopedia of Database Systems},
year="2018",
publisher="Springer International Publishing",
pages="1--6",
}

@book{lifschitz:2019,
  title={Answer set programming},
  author={Lifschitz, Vladimir},
  year={2019},
  publisher={Springer Heidelberg}
}



@inproceedings{Manh:2021,
  title={Towards autonomous semantic stream fusion for distributed video streams},
  author={Nguyen-Duc, Manh and Le-Tuan, Anh and Hauswirth, Manfred and Le-Phuoc, Danh},
  booktitle={Proceedings of the 15th ACM International Conference on Distributed and Event-based Systems},
  pages={172--175},
  year={2021}
}


@inproceedings{quigley2009ros,
  title={ROS: an open-source Robot Operating System},
  author={Quigley, Morgan and Conley, Ken and Gerkey, Brian and Faust, Josh and Foote, Tully and Leibs, Jeremy and Wheeler, Rob and Ng, Andrew Y and others},
  booktitle={ICRA workshop on open source software},
  volume={3},
  pages={5},
  year={2009},
  organization={Kobe, Japan}
}

@article{ros2:2018,
author = {Vincenzo DiLuoffo and William R Michalson and Berk Sunar},
title ={Robot Operating System 2: The need for a holistic security approach to robotic architectures},
journal = {International Journal of Advanced Robotic Systems},
volume = {15},
number = {3},
year = {2018},
}

@article{Armin:2019,
  author    = {Armin Haller and
               Krzysztof Janowicz and
               Simon J. D. Cox and
               Maxime Lefran{\c{c}}ois and
               Kerry Taylor and
               Danh Le Phuoc and
               Joshua Lieberman and
               Ra{\'{u}}l Garc{\'{\i}}a{-}Castro and
               Rob Atkinson and
               Claus Stadler},
  title     = {The modular {SSN} ontology: {A} joint {W3C} and {OGC} standard specifying
               the semantics of sensors, observations, sampling, and actuation},
  journal   = {Semantic Web},
  volume    = {10},
  number    = {1},
  pages     = {9--32},
  year      = {2019},
}

@article{lephuoc:2011,
  title={A native and adaptive approach for unified processing of linked streams and linked data},
  author={Le-Phuoc, Danh and Dao-Tran, Minh and Parreira, Josiane Xavier and Hauswirth, Manfred},
  journal={ISWC'11},
  year={2011}
}

@inproceedings{Daniele:2016,
  title={A query model to capture event pattern matching in RDF stream processing query languages},
  author={Dell’Aglio, Daniele and Dao-Tran, Minh and Calbimonte, Jean-Paul and Le Phuoc, Danh and Della Valle, Emanuele},
  booktitle={European Knowledge Acquisition Workshop},
  pages={145--162},
  year={2016},
  organization={Springer}
}

@InProceedings{Manh:2019,
author="Nguyen-Duc, Manh
and Le-Tuan, Anh
and Calbimonte, Jean-Paul
and Hauswirth, Manfred
and Le-Phuoc, Danh",
title="Autonomous RDF Stream Processing for IoT Edge Devices",
booktitle="Semantic Technology",
year="2019",
publisher="Springer",
address="Cham",
pages="304--319",
}

@ARTICLE{Wang:2020,
  title    = "{Multi-Sensor} Fusion in Automated Driving: A Survey",
  author   = "Wang, Z and Wu, Y and Niu, Q",
  journal  = "IEEE Access",
  volume   =  8,
  pages    = "2847--2868",
  year     =  2020,
}

@ARTICLE{Pendleton:2017,
  title     = "Perception, Planning, Control, and Coordination for Autonomous
               Vehicles",
  author    = "Pendleton, Scott Drew and Andersen, Hans and Du, Xinxin and
               Shen, Xiaotong and Meghjani, Malika and Eng, You Hong and Rus,
               Daniela and Ang, Marcelo H",
  journal   = "Machines",
  publisher = "Multidisciplinary Digital Publishing Institute",
  volume    =  5,
  number    =  1,
  pages     = "6",
  month     =  feb,
  year      =  2017,
  language  = "en"
}

@inproceedings{Daniel:2016,
  author    = {Daniel de Leng and
               Fredrik Heintz},
  title     = {DyKnow: {A} dynamically reconfigurable stream reasoning framework
               as an extension to the robot operating system},
  booktitle = {2016 {IEEE} International Conference on Simulation, Modeling, and
               Programming for Autonomous Robots, {SIMPAR} 2016},
  pages     = {55--60},
  publisher = {{IEEE}},
  year      = {2016},
}

@inproceedings{Daniel:2017,
  author    = {Daniel de Leng and
               Fredrik Heintz},
  title     = {Towards adaptive semantic subscriptions for stream reasoning in the
               robot operating system},
  booktitle = {2017 {IEEE/RSJ} International Conference on Intelligent Robots and
               Systems, {IROS} 2017},
  pages     = {5445--5452},
  publisher = {{IEEE}},
  year      = {2017},
}


@online{slam,
  author = {Cyrill Stachniss, Udo Frese, Giorgio Grisetti},
  title = {Open SLAM},
  url = {https://openslam.org},
  urldate = {2021-07-01}
}

@inproceedings{Bowman2020RobustAE,
  title={Robust and Efficient Semantic SLAM with Semantic Keypoints},
  author={S. Bowman and Kostas Daniilidis and George J. Pappas},
  year={2020}
}

@article{Dong:2020,
  author    = {Dongjiang Li and
               Xuesong Shi and
               Qiwei Long and
               Shenghui Liu and
               Wei Yang and
               Fangshi Wang and
               Qi Wei and
               Fei Qiao},
  title     = {{DXSLAM:} {A} Robust and Efficient Visual {SLAM} System with Deep
               Features},
  journal   = {CoRR},
  volume    = {abs/2008.05416},
  year      = {2020},
}
@article{Shuhuan:2021,
  author    = {Shuhuan Wen and
               Pengjiang Li and
               Yongjie Zhao and
               Hong Zhang and
               Fuchun Sun and
               Zhe Wang},
  title     = {Semantic visual {SLAM} in dynamic environment},
  journal   = {Autonomous Robots},
  volume    = {45},
  number    = {4},
  pages     = {493--504},
  year      = {2021},
}
@ARTICLE{Boccardi:2014,
  title     = "Five disruptive technology directions for {5G}",
  author    = "Boccardi, F and Heath, R W and Lozano, A and Marzetta, T L and
               Popovski, P",
  journal   = "IEEE Commun. Mag.",
  publisher = "ieeexplore.ieee.org",
  volume    =  52,
  number    =  2,
  pages     = "74--80",
  month     =  feb,
  year      =  2014,
}

@ARTICLE{Gui:2020,
  title     = "6G: Opening New Horizons for Integration of Comfort, Security, and Intelligence",
  author    = "Gui, G and Liu, M and Tang, F and Kato, N and Adachi, F",
  journal   = "IEEE Wirel. Commun.",
  publisher = "ieeexplore.ieee.org",
  volume    =  27,
  number    =  5,
  pages     = "126--132",
  month     =  oct,
  year      =  2020,
}

@ARTICLE{Viswanathan:2020,
  title     = "Communications in the {6G} Era",
  author    = "Viswanathan, Harish and Mogensen, Preben E",
  journal   = "IEEE Access",
  publisher = "Institute of Electrical and Electronics Engineers (IEEE)",
  volume    =  8,
  pages     = "57063--57074",
  year      =  2020
}

@ARTICLE{Kim:2015-hs,
  title    = "Multivehicle Cooperative Driving Using Cooperative Perception:
              Design and Experimental Validation",
  author   = "Kim, S and Qin, B and Chong, Z J and Shen, X and Liu, W and Ang,
              M H and Frazzoli, E and Rus, D",
  journal  = "IEEE Trans. Intell. Transp. Syst.",
  volume   =  16,
  number   =  2,
  pages    = "663--680",
  month    =  apr,
  year     =  2015,
}


@inproceedings{Rauch:2017,
  added-at = {2017-05-26T00:00:00.000+0200},
  author = {Rauch, Andreas and Klanner, Felix and Rasshofer, Ralph H. and Dietmayer, Klaus},
  booktitle = {Intelligent Vehicles Symposium},
  pages = {270-275},
  publisher = {IEEE},
  title = {Car2X-based perception in a high-level fusion architecture for cooperative perception systems.},
  year = 2012
}


@inproceedings{Chen:2019,
  title={Cooper: Cooperative perception for connected autonomous vehicles based on 3d point clouds},
  author={Chen, Qi and Tang, Sihai and Yang, Qing and Fu, Song},
  booktitle={2019 IEEE 39th International Conference on Distributed Computing Systems (ICDCS)},
  pages={514--524},
  year={2019},
  organization={IEEE}
}

@ARTICLE{Arnold:2020,
  title    = "Cooperative Perception for {3D} Object Detection in Driving
              Scenarios Using Infrastructure Sensors",
  author   = "Arnold, E and Dianati, M and de Temple, R and Fallah, S",
  journal  = "IEEE Trans. Intell. Transp. Syst.",
  pages    = "1--13",
  year     =  2020,
}

@INPROCEEDINGS{Rawashdeh:2018,
  title     = "Collaborative Automated Driving: A Machine Learning-based Method
               to Enhance the Accuracy of Shared Information",
  booktitle = "2018 21st International Conference on Intelligent Transportation
               Systems ({ITSC})",
  author    = "Rawashdeh, Z Y and Wang, Z",
  pages     = "3961--3966",
  month     =  nov,
  year      =  2018
}

 @InProceedings{Tsun-Hsuan:2020,
author="Wang, Tsun-Hsuan
and Manivasagam, Sivabalan
and Liang, Ming
and Yang, Bin
and Zeng, Wenyuan
and Urtasun, Raquel",

title="V2VNet: Vehicle-to-Vehicle Communication for Joint Perception and Prediction",
booktitle="Computer Vision -- ECCV 2020",
year="2020",
publisher="Springer International Publishing",
address="Cham",
pages="605--621",
}

@article{Moritz:2013,
  author    = {Moritz Tenorth and
               Michael Beetz},
  title     = {KnowRob: {A} knowledge processing infrastructure for cognition-enabled
               robots},
  journal   = {Int. J. Robotics Res.},
  volume    = {32},
  number    = {5},
  pages     = {566--590},
  year      = {2013},
}


@inproceedings{Mengtian:2020,
  title={Towards streaming image understanding},
  author={Li, Mengtian and Wang, Yu-Xiong and Ramanan, Deva},
  booktitle={European Conference on Computer Vision (ECCV)},
  year={2020}
}

@INPROCEEDINGS{Caveney:2012, 
author={D. Caveney and W. B. Dunbar}, 
booktitle={2012 IEEE Intelligent Vehicles Symposium}, 
title={Cooperative driving: Beyond V2V as an ADAS sensor}, 
year={2012}, 
volume={}, 
number={}, 
pages={529-534}, 
month={June},}


@INPROCEEDINGS{Sawade:2015, 
author={O. Sawade and I. Radusch}, 
booktitle={2015 IEEE 82nd Vehicular Technology Conference (VTC2015-Fall)}, 
title={Survey and Classification of Cooperative Automated Driver Assistance Systems}, 
year={2015}, 
volume={}, 
number={}, 
pages={1-5}, 
month={Sept},}

@article{Matthew:2019,
  author    = {Matthew O'Kelly and
               Varundev Sukhil and
               Houssam Abbas and
               Jack Harkins and
               Chris Kao and
               Yash Vardhan Pant and
               Rahul Mangharam and
               Dipshil Agarwal and
               Madhur Behl and
               Paolo Burgio and
               Marko Bertogna},
  title     = {{F1/10:} An Open-Source Autonomous Cyber-Physical Platform},
  journal   = {CoRR},
  volume    = {abs/1901.08567},
  year      = {2019},
}

@InProceedings{Keylly:2020,
  title = 	 {textsc{F1TENTH}: An Open-source Evaluation Environment for Continuous Control and Reinforcement Learning},
  author =       {O'Kelly, Matthew and Zheng, Hongrui and Karthik, Dhruv and Mangharam, Rahul},
  booktitle = 	 {Proceedings of the NeurIPS 2019 Competition and Demonstration Track},
  pages = 	 {77--89},
  year = 	 {2020},
  volume = 	 {123},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {08--14 Dec},
  publisher =    {PMLR},
}

@inproceedings{Minh:2017,
  author    = {Minh Dao{-}Tran and
               Thomas Eiter},
  editor    = {Carles Sierra},
  title     = {Streaming Multi-Context Systems},
  booktitle = {Proceedings of the Twenty-Sixth International Joint Conference on
               Artificial Intelligence, {IJCAI} 2017},
  pages     = {1000--1007},
  publisher = {ijcai.org},
  year      = {2017},
}

@article{Linda:2019,
  author    = {Linda van den Brink and
               Payam M. Barnaghi and
               Jeremy Tandy and
               Ghislain Atemezing and
               Rob Atkinson and
               Byron Cochrane and
               Yasmin Fathy and
               Ra{\'{u}}l Garc{\'{\i}}a{-}Castro and
               Armin Haller and
               Andreas Harth and
               Krzysztof Janowicz and
               Sefki Kolozali and
               Bart van Leeuwen and
               Maxime Lefran{\c{c}}ois and
               Joshua Lieberman and
               Andrea Perego and
               Danh Le Phuoc and
               Bill Roberts and
               Kerry Taylor and
               Rapha{\"{e}}l Troncy},
  title     = {Best practices for publishing, retrieving, and using spatial data
               on the web},
  journal   = {Semantic Web},
  volume    = {10},
  number    = {1},
  pages     = {95--114},
  year      = {2019},
}

@inproceedings{Le-Phuoc:2010,
  author    = {Danh Le-Phuoc and
               Josiane Xavier Parreira and
               Michael Hausenblas and
               Yuanbo Han and
               Manfred Hauswirth},
  title     = {Live linked open sensor database},
  booktitle = {{I-SEMANTICS}},
  publisher = {{ACM}},
  year      = {2010}
}

==> references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} If the citatiion in the text is numbered, the reference list should be arranged in ascending order. If the citation in the text is author/year, the reference list should be \textit{sorted} alphabetically and if there are several works by the same author, the following order should be used:
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer Nature style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O'Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}


==> sections.tex <==
\section{Section Heading}
\label{sec:1}
Use the template \emph{chapter.tex} together with the document class SVMono (monograph-type books) or SVMult (edited books) to style the various elements of your chapter content.

Instead of simply listing headings of different levels we recommend to let every heading be followed by at least a short passage of text.  Further on please use the \LaTeX\ automatism for all your cross-references and citations. And please note that the first line of text that follows a heading is not indented, whereas the first lines of all subsequent paragraphs are.

\section{Section Heading}
\label{sec:2}
% Always give a unique label
% and use \ref{<label>} for cross-references
% and \cite{<label>} for bibliographic references
% use \sectionmark{}
% to alter or adjust the section heading in the running head
Instead of simply listing headings of different levels we recommend to let every heading be followed by at least a short passage of text.  Further on please use the \LaTeX\ automatism for all your cross-references and citations.

Please note that the first line of text that follows a heading is not indented, whereas the first lines of all subsequent paragraphs are.

Use the standard \verb|equation| environment to typeset your equations, e.g.
%
\begin{equation}
a \times b = c\;,
\end{equation}
%
however, for multiline equations we recommend to use the \verb|eqnarray| environment\footnote{In physics texts please activate the class option \texttt{vecphys} to depict your vectors in \textbf{\itshape boldface-italic} type - as is customary for a wide range of physical subjects}.
\begin{eqnarray}
\left|\nabla U_{\alpha}^{\mu}(y)\right| &\le&\frac1{d-\alpha}\int
\left|\nabla\frac1{|\xi-y|^{d-\alpha}}\right|\,d\mu(\xi) =
\int \frac1{|\xi-y|^{d-\alpha+1}} \,d\mu(\xi)  \\
&=&(d-\alpha+1) \int\limits_{d(y)}^\infty
\frac{\mu(B(y,r))}{r^{d-\alpha+2}}\,dr \le (d-\alpha+1)
\int\limits_{d(y)}^\infty \frac{r^{d-\alpha}}{r^{d-\alpha+2}}\,dr
\label{eq:01}
\end{eqnarray}

\subsection{Subsection Heading}
\label{subsec:2}
Instead of simply listing headings of different levels we recommend to let every heading be followed by at least a short passage of text.  Further on please use the \LaTeX\ automatism for all your cross-references\index{cross-references} and citations\index{citations} as has already been described in Sect.~\ref{sec:2}.

\begin{quotation}
Please do not use quotation marks when quoting texts! Simply use the \verb|quotation| environment -- it will automatically be rendered in line with the preferred layout.
\end{quotation}


\subsubsection{Subsubsection Heading}
Instead of simply listing headings of different levels we recommend to let every heading be followed by at least a short passage of text.  Further on please use the \LaTeX\ automatism for all your cross-references and citations as has already been described in Sect.~\ref{subsec:2}, see also Fig.~\ref{fig:1}\footnote{If you copy text passages, figures, or tables from other works, you must obtain \textit{permission} from the copyright holder (usually the original publisher). Please enclose the signed permission with the manuscript. The sources\index{permission to print} must be acknowledged either in the captions, as footnotes or in a separate section of the book.}

Please note that the first line of text that follows a heading is not indented, whereas the first lines of all subsequent paragraphs are.

% For figures use
%
\begin{figure}[b]
\sidecaption
% Use the relevant command for your figure-insertion program
% to insert the figure file.
% For example, with the graphicx style use
\includegraphics[scale=.65]{figure}
%
% If no graphics program available, insert a blank space i.e. use
%\picplace{5cm}{2cm} % Give the correct figure height and width in cm
%
\caption{If the width of the figure is less than 7.8 cm use the \texttt{sidecapion} command to flush the caption on the left side of the page. If the figure is positioned at the top of the page, align the sidecaption with the top of the figure -- to achieve this you simply need to use the optional argument \texttt{[t]} with the \texttt{sidecaption} command}
\label{fig:1}       % Give a unique label
\end{figure}


\paragraph{Paragraph Heading} %
Instead of simply listing headings of different levels we recommend to let every heading be followed by at least a short passage of text.  Further on please use the \LaTeX\ automatism for all your cross-references and citations as has already been described in Sect.~\ref{sec:2}.

Please note that the first line of text that follows a heading is not indented, whereas the first lines of all subsequent paragraphs are.

For typesetting numbered lists we recommend to use the \verb|enumerate| environment -- it will automatically rendered in line with the preferred layout.

\begin{enumerate}
\item{Livelihood and survival mobility are oftentimes coutcomes of uneven socioeconomic development.}
\begin{enumerate}
\item{Livelihood and survival mobility are oftentimes coutcomes of uneven socioeconomic development.}
\item{Livelihood and survival mobility are oftentimes coutcomes of uneven socioeconomic development.}
\end{enumerate}
\item{Livelihood and survival mobility are oftentimes coutcomes of uneven socioeconomic development.}
\end{enumerate}


\subparagraph{Subparagraph Heading} In order to avoid simply listing headings of different levels we recommend to let every heading be followed by at least a short passage of text. Use the \LaTeX\ automatism for all your cross-references and citations as has already been described in Sect.~\ref{sec:2}, see also Fig.~\ref{fig:2}.

For unnumbered list we recommend to use the \verb|itemize| environment -- it will automatically be rendered in line with the preferred layout.

\begin{itemize}
\item{Livelihood and survival mobility are oftentimes coutcomes of uneven socioeconomic development, cf. Table~\ref{tab:1}.}
\begin{itemize}
\item{Livelihood and survival mobility are oftentimes coutcomes of uneven socioeconomic development.}
\item{Livelihood and survival mobility are oftentimes coutcomes of uneven socioeconomic development.}
\end{itemize}
\item{Livelihood and survival mobility are oftentimes coutcomes of uneven socioeconomic development.}
\end{itemize}

\begin{figure}[t]
\sidecaption[t]
% Use the relevant command for your figure-insertion program
% to insert the figure file.
% For example, with the option graphics use
\includegraphics[scale=.65]{figure}
%
% If no graphics program available, insert a blank space i.e. use
%\picplace{5cm}{2cm} % Give the correct figure height and width in cm
%
%\caption{Please write your figure caption here}
\caption{If the width of the figure is less than 7.8 cm use the \texttt{sidecapion} command to flush the caption on the left side of the page. If the figure is positioned at the top of the page, align the sidecaption with the top of the figure -- to achieve this you simply need to use the optional argument \texttt{[t]} with the \texttt{sidecaption} command}
\label{fig:2}       % Give a unique label
\end{figure}

\runinhead{Run-in Heading Boldface Version} Use the \LaTeX\ automatism for all your cross-references and citations as has already been described in Sect.~\ref{sec:2}.

\subruninhead{Run-in Heading Boldface and Italic Version} Use the \LaTeX\ automatism for all your cross-refer\-ences and citations as has already been described in Sect.~\ref{sec:2}\index{paragraph}.

\subsubruninhead{Run-in Heading Displayed Version} Use the \LaTeX\ automatism for all your cross-refer\-ences and citations as has already been described in Sect.~\ref{sec:2}\index{paragraph}.
% Use the \index{} command to code your index words
%
% For tables use
%
\begin{table}[!t]
\caption{Please write your table caption here}
\label{tab:1}       % Give a unique label
%
% Follow this input for your own table layout
%
\begin{tabular}{p{2cm}p{2.4cm}p{2cm}p{4.9cm}}
\hline\noalign{\smallskip}
Classes & Subclass & Length & Action Mechanism  \\
\noalign{\smallskip}\svhline\noalign{\smallskip}
Translation & mRNA$^a$  & 22 (19--25) & Translation repression, mRNA cleavage\\
Translation & mRNA cleavage & 21 & mRNA cleavage\\
Translation & mRNA  & 21--22 & mRNA cleavage\\
Translation & mRNA  & 24--26 & Histone and DNA Modification\\
\noalign{\smallskip}\hline\noalign{\smallskip}
\end{tabular}
$^a$ Table foot note (with superscript)
\end{table}
%
\section{Section Heading}
\label{sec:3}
% Always give a unique label
% and use \ref{<label>} for cross-references
% and \cite{<label>} for bibliographic references
% use \sectionmark{}
% to alter or adjust the section heading in the running head
Instead of simply listing headings of different levels we recommend to let every heading be followed by at least a short passage of text.  Further on please use the \LaTeX\ automatism for all your cross-references and citations as has already been described in Sect.~\ref{sec:2}.

Please note that the first line of text that follows a heading is not indented, whereas the first lines of all subsequent paragraphs are.

If you want to list definitions or the like we recommend to use the enhanced \verb|description| environment -- it will automatically rendered in line with the preferred layout.

\begin{description}[Type 1]
\item[Type 1]{That addresses central themes pertainng to migration, health, and disease. In Sect.~\ref{sec:1}, Wilson discusses the role of human migration in infectious disease distributions and patterns.}
\item[Type 2]{That addresses central themes pertainng to migration, health, and disease. In Sect.~\ref{subsec:2}, Wilson discusses the role of human migration in infectious disease distributions and patterns.}
\end{description}

\subsection{Subsection Heading} %
In order to avoid simply listing headings of different levels we recommend to let every heading be followed by at least a short passage of text. Use the \LaTeX\ automatism for all your cross-references and citations citations as has already been described in Sect.~\ref{sec:2}.

Please note that the first line of text that follows a heading is not indented, whereas the first lines of all subsequent paragraphs are.

\begin{svgraybox}
If you want to emphasize complete paragraphs of texts we recommend to use the newly defined class option \verb|graybox| and the newly defined environment \verb|svgraybox|. This will produce a 15 percent screened box 'behind' your text.

If you want to emphasize complete paragraphs of texts we recommend to use the newly defined class option and environment \verb|svgraybox|. This will produce a 15 percent screened box 'behind' your text.
\end{svgraybox}


\subsubsection{Subsubsection Heading}
Instead of simply listing headings of different levels we recommend to let every heading be followed by at least a short passage of text.  Further on please use the \LaTeX\ automatism for all your cross-references and citations as has already been described in Sect.~\ref{sec:2}.

Please note that the first line of text that follows a heading is not indented, whereas the first lines of all subsequent paragraphs are.

\begin{theorem}
Theorem text goes here.
\end{theorem}
%
% or
%
\begin{definition}
Definition text goes here.
\end{definition}

\begin{proof}
%\smartqed
Proof text goes here.
%\qed
\end{proof}

\paragraph{Paragraph Heading} %
Instead of simply listing headings of different levels we recommend to let every heading be followed by at least a short passage of text.  Further on please use the \LaTeX\ automatism for all your cross-references and citations as has already been described in Sect.~\ref{sec:2}.

Note that the first line of text that follows a heading is not indented, whereas the first lines of all subsequent paragraphs are.
%
% For built-in environments use
%
\begin{theorem}
Theorem text goes here.
\end{theorem}
%
\begin{definition}
Definition text goes here.
\end{definition}
%
\begin{proof}
%\smartqed
Proof text goes here.
%\qed
\end{proof}
%
\begin{trailer}{Trailer Head}
If you want to emphasize complete paragraphs of texts in an \verb|Trailer Head| we recommend to
use  \begin{verbatim}\begin{trailer}{Trailer Head}
...
\end{trailer}\end{verbatim}
\end{trailer}
%
\begin{question}{Questions}
If you want to emphasize complete paragraphs of texts in an \verb|Questions| we recommend to
use  \begin{verbatim}\begin{question}{Questions}
...
\end{question}\end{verbatim}
\end{question}
\eject%
\begin{important}{Important}
If you want to emphasize complete paragraphs of texts in an \verb|Important| we recommend to
use  \begin{verbatim}\begin{important}{Important}
...
\end{important}\end{verbatim}
\end{important}
%
\begin{warning}{Attention}
If you want to emphasize complete paragraphs of texts in an \verb|Attention| we recommend to
use  \begin{verbatim}\begin{warning}{Attention}
...
\end{warning}\end{verbatim}
\end{warning}

\begin{programcode}{Program Code}
If you want to emphasize complete paragraphs of texts in an \verb|Program Code| we recommend to
use

\verb|\begin{programcode}{Program Code}|

\verb|\begin{verbatim}...\end{verbatim}|

\verb|\end{programcode}|

\end{programcode}
%
\begin{tips}{Tips}
If you want to emphasize complete paragraphs of texts in an \verb|Tips| we recommend to
use  \begin{verbatim}\begin{tips}{Tips}
...
\end{tips}\end{verbatim}
\end{tips}
\eject
%
\begin{overview}{Overview}
If you want to emphasize complete paragraphs of texts in an \verb|Overview| we recommend to
use  \begin{verbatim}\begin{overview}{Overview}
...
\end{overview}\end{verbatim}
\end{overview}
\begin{backgroundinformation}{Background Information}
If you want to emphasize complete paragraphs of texts in an \verb|Background|
\verb|Information| we recommend to
use

\verb|\begin{backgroundinformation}{Background Information}|

\verb|...|

\verb|\end{backgroundinformation}|
\end{backgroundinformation}
\begin{legaltext}{Legal Text}
If you want to emphasize complete paragraphs of texts in an \verb|Legal Text| we recommend to
use  \begin{verbatim}\begin{legaltext}{Legal Text}
...
\end{legaltext}\end{verbatim}
\end{legaltext}
